Probing Anisotropies of the Stochastic Gravitational Wave Background with LISA

We investigate the sensitivity of the Laser Interferometer Space Antenna (LISA) to the anisotropies of the Stochastic Gravitational Wave Background (SGWB). We first discuss the main astrophysical and cosmological sources of SGWB which are characterized by anisotropies in the GW energy density, and we build a Signal-to-Noise estimator to quantify the sensitivity of LISA to different multipoles. We then perform a Fisher matrix analysis of the prospects of detectability of anisotropic features with LISA for individual multipoles, focusing on a SGWB with a power-law frequency profile. We compute the noise angular spectrum taking into account the specific scan strategy of the LISA detector. We analyze the case of the kinematic dipole and quadrupole generated by Doppler boosting an isotropic SGWB. We find that $\beta\, \Omega_{\rm GW}\sim 2\times 10^{-11}$ is required to observe a dipolar signal with LISA. The detector response to the quadrupole has a factor $\sim 10^3 \,\beta$ relative to that of the dipole. The characterization of the anisotropies, both from a theoretical perspective and from a map-making point of view, allows us to extract information that can be used to understand the origin of the SGWB, and to discriminate among distinct superimposed SGWB sources.

==> Detection.tex <==
Sachiko

==> Response.tex <==


Arianna, Carlo, Mauro, Angelo, Chiara,  Giulia, Lorenzo, Valerie, Sachiko, Marco, Tristan, Nicola Bartolo, Caner, Robert Caldwell, Gianmassimo 
\\


Plane wave expansion for the metric perturbation $h_{ij}(t,\vec x)$ produced by a stochastic background:
\begin{equation}
h_{ij}(t,\vec x) = \sum_{\lambda} \int_{-\infty}^\infty \!\!\!\!df\ \int 
d^2 \hat n\ h_{\lambda}(f,\hat n)\ e^{i2\pi f(t-\hat n\cdot\vec x)}\ 
e_{ij}^{\lambda}(\hat n)\ ,
\label{e:h_ab}
\end{equation}



The signal in one LISA interferometer channel can be written as 
\begin{equation}
s_{12} \left( t \right) -n_1 \left(t,\vec x_1 \right) = \frac{L}{2}\hat{l}_{12}^a \hat{l}_{12}^b  \sum_\lambda  \int_{-\infty}^{\infty} {d f} {\rm e}^{i 2 \pi f (t-L)} \int d^2 \hat{n}\, e^{-2\pi i f\hat{n}\cdot \vec{x}_{1}}  e_{ab,\lambda}\left(\hat{n}\right)\, h_\lambda\left(f, \hat{n}\right) \mathcal{T}\left(f \,L, \hat{n}\cdot \hat{l}_{12}\right)
\end{equation}
where we have defined  the detector transfer function 
%
\begin{equation}
 \mathcal{T}\left(f \,L, \hat{n}\cdot \hat{l}_{12}\right)\equiv e^{-\pi i f L \left[ 1 + \hat{n}\cdot\hat{l}_{12}\right]} \frac{\sin\left(\pi f L \left[ 1 - \hat{n}\cdot\hat{l}_{12}\right] \right)}{\pi f L \left[ 1 - \hat{n}\cdot\hat{l}_{12}\right]}  +   e^{\pi i f L \left[ 1 - \hat{n}\cdot\hat{l}_{12}\right]} \frac{\sin\left(\pi f L \left[ 1 + \hat{n}\cdot\hat{l}_{12}\right] \right)}{\pi f L \left[ 1 +\hat{n}\cdot\hat{l}_{12}\right]}   
\end{equation}

Now we define the three LISA X,Y,Z interferometers

\begin{eqnarray}
s_1-n_1 \equiv \sigma_X &\propto& \left( {\rm time \; } \vec{x}_1 \rightarrow \vec{x}_2 \rightarrow \vec{x}_1 \right) -  \left( {\rm time \; } \vec{x}_1 \rightarrow \vec{x}_3 \rightarrow \vec{x}_1 \right) \nonumber\,,\\ 
s_2-n_2  \equiv \sigma_Y &\propto& \left( {\rm time \; } \vec{x}_2 \rightarrow \vec{x}_3 \rightarrow \vec{x}_2 \right) -  \left( {\rm time \; } \vec{x}_2 \rightarrow \vec{x}_1 \rightarrow \vec{x}_2 \right) \nonumber\,,\\ 
s_3-n_3\equiv \sigma_Z &\propto& \left( {\rm time \; } \vec{x}_3 \rightarrow \vec{x}_1 \rightarrow \vec{x}_3 \right) -  \left( {\rm time \; } \vec{x}_3 \rightarrow \vec{x}_2 \rightarrow \vec{x}_3 \right)  \,.  
\label{sigma-123} 
\end{eqnarray} 

or, in a more compact way,

\begin{equation}
s_i-n_i	 = \left({\rm time }\;\; \vec{x}_{i}\rightarrow\vec{x}_{i+1}\rightarrow\vec{x}_{i}\right)\; \; - \;\;  \left({\rm time }\;\; \vec{x}_{i}\rightarrow\vec{x}_{i+2}\rightarrow\vec{x}_{i}\right)
\end{equation}
where the vertices are defined modulo $2$  (namely  $\vec{x}_{4}=\vec{x}_{1}$ and $\vec{x}_{5}=\vec{x}_{2}$)\\Now, can define the arm directions as 
\begin{equation} 
\frac{(\vec{x}_2 - \vec{x}_1)}{L} =  \hat l_{21}  \equiv  {\hat U}_1 \;\;\;,\;\;\; 
\frac{(\vec{x}_3 - \vec{x}_2)}{L} =  \hat l_{32}\equiv {\hat U}_2  \;\;\;,\;\;\; 
\frac{(\vec{x}_1 - \vec{x}_3)}{L} =  \hat l_{13}\equiv  {\hat U}_3  \;, 
\label{LISA-arms} 
\end{equation}
and the signal can be written as  (I neglect the noise for the moment)
\begin{equation}
\sigma_{i} \left( t \right) \equiv s_i(t)-n_i (t)  = L  \sum_\lambda  \int_{-\infty}^{\infty} {d f} {\rm e}^{i 2 \pi f (t-L)} \int d^2 \hat{n}\, \frac{1}{2}\,e^{-2\pi i f \hat{n}\cdot \vec{x}_{i}(t)}  \, h_\lambda\left(f, \hat{n}\right) Q^{i}_{ab,\lambda}\left(t,f, \hat{n}\right)
\end{equation}

where we have introduced the function
\begin{eqnarray} 
{\cal Q}^i_{\lambda}  \left(t, f, \hat{n} \right) &\equiv&  e_{ab,\lambda}\left(\hat{n}\right)
\,  \left[  {\cal T} \left( f L ,\, {\hat n} \cdot {\hat U}^i (t) \right) {\hat U}_a^i (t){\hat U}_b^i 
(t)-   {\cal T} \left( f L ,\, - {\hat n} \cdot {\hat U}^{i+2}(t) \right) {\hat U}_a^{i+2}(t) {\hat U}_b^{i+2}(t) \right]\;, \nonumber\\ 
\end{eqnarray}
where it is important to take into account the dependence on time, due to the motion of the satellites.
The standard LISA output channels $A$, $E$ and $T$ are constructed as 
%
\begin{eqnarray} 
 \sigma_A &=& \frac{1}{3} \left( 2 \sigma_X - \sigma_Y - \sigma_Z \right) \;, 
\nonumber\\ 
\sigma_E &=& \frac{1}{\sqrt{3}} \left( \sigma_Z - \sigma_Y \right)  \;, 
\nonumber\\ 
\sigma_T &=&  \frac{1}{3} \left( \sigma_X + \sigma_Y + \sigma_Z \right)  \;. 
\label{signal-AET}
\end{eqnarray} 
%
so if we want to obtain the signal in these three standard channels we introduce the matrix $c$  given by 
%
\begin{equation}
c =  \begin{pmatrix}
\tfrac{2}{3} & - \tfrac{1}{3} & - \tfrac{1}{3}  \\[5pt]
0 & - \tfrac{1}{\sqrt{3}}  &  \tfrac{1}{\sqrt{3}} \\[5pt]
\tfrac{1}{3} & \tfrac{1}{3} & \tfrac{1}{3} 
\end{pmatrix} \;. 
\label{matrix-c}
\end{equation}  
and we have 

%
\begin{equation} 
\sigma_O(t) =  L  \sum_\lambda  \int_{-\infty}^{\infty} {d f} {\rm e}^{i 2 \pi f (t-L)} \int d^2 \hat{n}\, \frac{1}{2}\,e^{-2\pi i\hat{n}\cdot \vec{x}_{i}(t)}  \, h_\lambda\left(f, \hat{n}\right) c_{Oi} Q^{i}_{\lambda}\left(t,f, \hat{n}\right)
\label{Sigma-O}
\end{equation} 
%

where ${ O} = \{ A,E,T \}$.\\
Now, we Fourier transform the signal by integrating 	over a time interval $\tau$ centered at $t$
\begin{equation}
\sigma_{O}\left(t,f\right)=\int_{t-\tau/2}^{t+\tau/2} d t'  {\rm e}^{-2\pi i f t'} \sigma_{O}\left(t'\right)
\end{equation}

The integral is done on a timescale much smaller than that controlling the motion of the satellites, so we can assume $Q$ as constant, and we have 

%
\begin{eqnarray} 
\sigma_O\left(f,t\right) &\simeq & L  \sum_\lambda  \int_{-\infty}^{\infty} {d f'}   \int_{t-\tau/2}^{t+\tau/2} d t'   {\rm e}^{- 2 \pi i  (f-f')t'}  {\rm e}^{- 2 \pi i L f' } \int d^2 \hat{n}\, \frac{1}{2}\,e^{-2\pi i f' \hat{n}\cdot \vec{x}_{i}(t')}  \, h_\lambda\left(f', \hat{n}\right) c_{Oi} Q^{i}_{\lambda}\left(t',f', \hat{n}\right)\nonumber\\
&\simeq &  L  \sum_\lambda  \int_{-\infty}^{\infty} {d f'}    {\rm e}^{- 2 \pi i  (f-f')t}  \frac{{\rm sin}\left(\left(f-f'\right)\pi \tau\right)}{\left(f-f'\right)\pi }    {\rm e}^{- 2 \pi i L f' } \frac{1}{2}\int d^2 \hat{n}\,e^{-2\pi i f' \hat{n}\cdot \vec{x}_{i}(t)}  \, h_\lambda\left(f', \hat{n}\right) c_{Oi} Q^{i}_{\lambda}\left(t,f', \hat{n}\right)\nonumber\\
\label{SigmaF2}
\end{eqnarray} 
%
We define 
\begin{equation}
\delta_{\tau}\left(f-f'\right)\equiv  \frac{{\rm sin}\left(\left(f-f'\right)\pi \tau\right)}{\left(f-f'\right)\pi } \,,
\end{equation}
which has the following properties
\begin{equation}
\lim_{\tau\rightarrow\infty}\delta_{\tau} \left(f-f'\right) =\delta \left(f-f'\right)
\end{equation}
and we have 
%
\begin{eqnarray} 
\frac{\sigma_O\left(f,t\right)}{L} &\simeq &   \sum_\lambda  \int_{-\infty}^{\infty} {d f'}    {\rm e}^{- 2 \pi i  (f-f')t}   \delta_{\tau} \left(f-f'\right)  {\rm e}^{- 2 \pi i L f' } \int d^2 \hat{n}\, \frac{1}{2}\,e^{-2\pi i f' \hat{n}\cdot \vec{x}_{i}(t)}  \, h_\lambda\left(f', \hat{n}\right) \tilde{ Q}^{i}_{\lambda}\left(t,f', \hat{n}\right)
\label{SigmaF3}
\end{eqnarray} 
%
where we have redefined $\tilde{ Q}^{i}_{\lambda}\left(t',f', \hat{n}\right)\equiv c_{Oi} Q^{i}_{\lambda}\left(t,f', \hat{n}\right)$. Now we can compute the two-point correlator
\begin{eqnarray}
\left\langle \sigma_O^*  \left(f, t \right)   \sigma_{O'} \left( f',t' \right) \right\rangle &=&\sum_{\lambda\lambda'} \int_{-\infty}^{\infty} {d f_1}  \int_{-\infty}^{\infty} {d f_2}  \int d^2 \hat{n}  \int d^2 \hat{n}'  {\rm e}^{ 2 \pi i  (f-f_1)t}  {\rm e}^{ -2 \pi i  (f'-f_2)t'} {\rm e}^{ 2 \pi i L f_1 } {\rm e}^{ -2 \pi i L f_2 }  \nonumber\\ 
&\times&\delta_{\tau} \left(f-f_1\right)  \delta_{\tau} \left(f'-f_2\right)\frac{1}{4} \tilde{ Q}^{O*}_{\lambda}\left(t,f_1, \hat{n}\right)\tilde{ Q}^{O'}_{\lambda'}\left(t',f_2, \hat{n}'\right) e^{2\pi i f_1 \hat{n}\cdot \vec{x}_{O}(t)}  e^{-2\pi i f_2 \hat{n}' \cdot \vec{x}_{O'}(t')} \nonumber\\ 
&\times&  \left \langle \tilde{h}_{\lambda}^* \left( f_1 ,\, \hat{n} \right) \tilde{h}_{\lambda'} \left( f_2 ,\, \hat{n}' \right) \right\rangle
\end{eqnarray}
Now we can use the following ansatz for the two point correlator of the GW 
\begin{equation}
\left\langle \tilde{h}_{\lambda}^*\left(f_1, \hat{n}\right)  \tilde{h}_{\lambda'}\left(f_2, \hat{n}'\right)\right\rangle =\frac{1}{2} \delta\left(f_1-f_2\right)\frac{\delta^{(2)}\left(\hat{n}-\hat{n}'\right)}{4 \pi} S_{h}\left(|f_1|, \hat{n}\right) \delta_{\lambda \lambda'}
\label{2point}
\end{equation}
where $S_{h}\left(f, \hat{n}\right)$ is the power spectral density of gravitational waves, and it has not been assumed isotropic. 
The correlator becomes
\begin{eqnarray}
\left\langle \sigma_O^*  \left(f, t \right)   \sigma_{O'} \left( f',t' \right) \right\rangle &=&\sum_{\lambda\lambda'} \int_{-\infty}^{\infty} {d f_1}  \int_{-\infty}^{\infty} {d f_2}  \int d^2 \hat{n}  \int d^2 \hat{n}'  {\rm e}^{ 2 \pi i  (f-f_1)t}  {\rm e}^{ -2 \pi i  (f'-f_2)t'} {\rm e}^{ 2 \pi i L f_1 } {\rm e}^{ -2 \pi i L f_2 }  \nonumber\\ 
&\times&\delta_{\tau} \left(f-f_1\right)  \delta_{\tau} \left(f'-f_2\right)\frac{1}{4} \tilde{ Q}^{O*}_{\lambda}\left(t,f_1, \hat{n}\right)\tilde{ Q}^{O'}_{\lambda'}\left(t',f_2, \hat{n}'\right) e^{2\pi i f_1 \hat{n}\cdot \vec{x}_{O}(t)}  e^{-2\pi i f_2 \hat{n}' \cdot \vec{x}_{O'}(t')} \nonumber\\ 
&\times& \frac{1}{2} \delta\left(f_1-f_2\right)\frac{\delta^{(2)}\left(\hat{n}-\hat{n}'\right)}{4 \pi} S_{h}\left(|f_1|, \hat{n}\right) \delta_{\lambda \lambda'}
\end{eqnarray}
We perform the integration on $d f_2$ and $d^2\hat{n}'$ and we obtain
\begin{eqnarray}
\left\langle \sigma_O^*  \left(f, t \right)   \sigma_{O'} \left( f',t' \right) \right\rangle &=&\sum_{\lambda} \int_{-\infty}^{\infty} {d f_1}   \int d^2 \hat{n}  \, {\rm e}^{ -2 \pi i  f_1(t-t')}  {\rm e}^{ 2 \pi i  (f t-f' t')} \delta_{\tau} \left(f-f_1\right)  \delta_{\tau} \left(f'-f_2\right) \nonumber\\ 
&\times&\frac{1}{4} \tilde{ Q}^{O*}_{\lambda}\left(t,f_1, \hat{n}\right)\tilde{ Q}^{O'}_{\lambda}\left(t',f_1, \hat{n}\right) e^{2\pi i f_1 \hat{n}\cdot \left(\vec{x}_{O}(t)  -  \vec{x}_{O'}(t')\right) } \frac{1}{8\pi} S_{h}\left(|f_1|, \hat{n}\right) 
\end{eqnarray}
Now we assume $f=f'$ and $t=t'$ and we use the property
\begin{equation}
\delta_{\tau}\left(f-f_1\right) \delta_{\tau}\left(f-f_1\right)\simeq \tau \,\delta\left(f-f_1\right)
\end{equation}
and we integrate over $df_1$ obtaining 
\begin{eqnarray}
\left\langle \sigma_O^*  \left(f, t \right)   \sigma_{O'} \left( f,t \right) \right\rangle &=&\frac{\tau}{2}\sum_{\lambda}  \int d^2 \hat{n}\left[ \frac{1}{4} \tilde{ Q}^{O*}_{\lambda}\left(t,f, \hat{n}\right)\tilde{ Q}^{O'}_{\lambda}\left(t,f, \hat{n}\right) e^{2\pi i f \hat{n}\cdot \left(\vec{x}_{O}(t)  -  \vec{x}_{O'}(t)\right) }   \right] S_{h}\left(|f|, \hat{n}\right) \nonumber\\
\end{eqnarray}
This expression can be rewritten as
\begin{eqnarray}
\left\langle \sigma_O^*  \left(f, t \right)   \sigma_{O'} \left( f,t \right) \right\rangle &=&\frac{\tau}{2}\sum_{\lambda}  \int d^2 \hat{n}\,\mathcal{R}_{OO'}^{\lambda}\left(t,f, \hat{n}\right)  S_{h}\left(|f|, \hat{n}\right) 
\end{eqnarray}
where
\begin{equation}
\mathcal{R}_{OO'}^{\lambda}\left(t,f, \hat{n}\right) \equiv \frac{1}{4} e^{2\pi i f \hat{n}\cdot \left(\vec{x}_{O}\left(t\right)  -  \vec{x}_{O'}\left(t\right)\right) }  \tilde{ Q}^{O*}_{\lambda}\left(t,f, \hat{n}\right)\tilde{ Q}^{O'}_{\lambda}\left(t,f, \hat{n}\right) 
\end{equation}
Now we can expand the response function and the SGWB power spectrum density into spherical harmonics. In particular we first factorize the spectral density as
\begin{equation}
S_{h}\left(|f|, \hat{n}\right)= S\left(f\right) P\left(\hat{n}\right)
\end{equation}
and then we expand the spatial part  in  spherical harmonics as
\begin{equation}
 P\left(\hat{n}\right)=\sum_{\ell m } p_{\ell m }\,  Y_{\ell m }\left(\hat{n}\right)
\end{equation}
In the same way we decompose the response function

\begin{equation}
\mathcal{R}_{OO'}^{\lambda}\left(t,f, \hat{n}\right) =\sum_{\ell m } r_{\ell m }^{OO'} \left(t, f\right) Y_{\ell m }\left(\hat{n}\right)
\end{equation}
So the two-point correlator become
\begin{eqnarray}
\mathcal{S}_{OO'}&\equiv&\frac{\tau}{2} \left\langle \sigma_O^*  \left(f, t \right)   \sigma_{O'} \left( f,t \right) \right\rangle\nonumber\\
&=& \frac{\tau}{2}  \int d^2 \hat{n}\,\sum_{\ell m } r_{\ell m }^{OO'} \left(t, f\right)   \sum_{\ell' m' } p_{\ell' m' } \left(f\right) Y_{\ell m }\left(\hat{n}\right) Y_{\ell' m' }\left(\hat{n}\right)
\end{eqnarray}
and using the properties of the spherical harmonics

\begin{eqnarray}
\mathcal{S}_{OO'}= \frac{\tau}{2} S(f) \,\sum_{\ell m } r_{\ell m }^{OO'} \left(t, f\right)\,   p_{\ell m} 
\end{eqnarray}

\subsection{Sensitivity of response function to direction}

We start from 
\begin{equation}
\mathcal{R}_{OO'}^{\lambda}\left(t,f, \hat{n}\right) =\sum_{\ell m } r_{\ell m }^{OO'} \left(t, f\right) Y_{\ell m }\left(\hat{n}\right)
\end{equation}
and we invert it to find the multipole
\begin{equation}
 r_{\ell m }^{OO'} \left(t, f\right) = \int d^2 \hat{n} \, \mathcal{R}_{OO'}^{\lambda}\left(t,f, \hat{n}\right) Y_{\ell m }^* \left(\hat{n}\right)
\end{equation}
This quantity depends on the coordinate system chosen for the detector, but we can define a quantity invariant under a rotation of the coordinate system (like the $C_{\ell}$), taking the square of the previous quantity
\begin{equation}
\mathcal{C}_{\ell}(f,t )=\frac{1}{2\ell +1}\sum_{m=-\ell}^{\ell} |r_{\ell m }^{OO'}\left(t, f\right)  |^2
\end{equation}
From this quantity, having the response function of the detector, we can compute the dependence from the angular scales $(\ell)$ and frequency.


